What if CLIQUE were fast? Maximum Cliques in Information Networks and Strong Components in Temporal Networks

Exact maximum clique finders have progressed to the point where we can investigate cliques in million-node social and information networks, as well as find strongly connected components in temporal networks. We use one such finder to study a large collection of modern networks emanating from biological, social, and technological domains. We show inter-relationships between maximum cliques and several other common network properties, including network density, maximum core, and number of triangles. In temporal networks, we find that the largest temporal strong components have around 20-30% of the vertices of the entire network. These components represent groups of highly communicative individuals. In addition, we discuss and improve the performance and utility of the maximum clique finder itself.

==> scratch.tex <==
%todo: make these visualizations consistent
\def \lentab{2.5in}
\begin{figure*}[t!]
\centering
    \hspace{0mm}\subfigure[Reality]
    	{\label{fig:tscc-reality}\includegraphics[width=3in]{images/reality_tscc_best_sm2.png}}
    \hspace{-0mm}\subfigure[Retweets]
    	{\label{fig:tscc-retweets}\includegraphics[width=3in]{images/retweet_tscc_induced1_sm.png}}
%    \hspace{-0mm}\subfigure[Twitter Copen]
%    	{\label{fig:tscc-twittercop}\includegraphics[width=3in]{images/twittercop_tscc_induced1_sm.png}}
    	\vspace{-3mm}
  \caption{\textbf{Largest Temporal Strongly Connected Component.} The Largest TSCC are induced from each of the original graphs. 
  (a) From the largest TSCC in the reality call graph, we see a lot of small stars, indicating that one individual communicates with many others that don't communicate much with anyone else. It is clear that the low degree vertices are important as they act as temporal bridges allowing for the communication of information across distinct stars and communities. (b) In the political retweet network, there are a few extremely active users who consistently retweet... (todo: get better visualization of retweets, using consistent color scales) }
  \label{fig:loss}
\end{figure*}



\def \lentab{2.5in}
\begin{figure*}[t!]
\centering
    \hspace{0mm}\subfigure[Infectious Contact Network (Dublin)]
    	{\label{fig:reach-infectious}\includegraphics[width=3in]{images/infectious-dublin-reachRs-groups-sm.png}}
    \hspace{-0mm}\subfigure[Retweet Network]
    	{\label{fig:reach-retweets}\includegraphics[width=3in]{images/retweet-2parties-Rs-sm.png}}
  \caption{\textbf{Temporal Reachability Graphs.} These graphs reveal community structures based on temporal connectivity that are not as strong as in the original data. In the political retweet network, we see two communities which indicate the political parties. for the retweet network and the infectious contact network from the Dublin museum of science. (todo: fix explanation)}
%The colors represent degree, going from yellow (lowest degree), to green, to blue, to purple/red being the max. (all colors sort of evenly distributed from min degree to max)
%So the edges in this graph represent reciprocal temporal paths between two vertices... 
%From the reachability graph we see these two political parties who are very well temporally connected within their own political party, but have "relatively" sparse temporal connectivity between political parties.
%Whereas the temporal SCC (max clique of the vertices in the visualization) corresponds to only one of the political parties (??what does this mean? We might be able to come up with a nice story here.)}
%
%That visualization appears to be of only a single party, since we didn't see these two groups arise.. What I meant is that the TSCC appears to be from only one party (although we'd have to verify), whereas in the strong temporal reachability graph (this new visualization) we clearly see two parties... Sorry for the previous unclear email, got excited and didn't think enough on how to explain it properly.
%
%some of these temporal reachability graphs are strikingly different, see the other one I attached. This is from the dublin infectious contact network. It seems to form these dense groups all connected together usually by low-degree nodes... Not yet sure how to interpret this one with respect to the actual data/collection. But since the network is from the Dublin Museum of Science over two weeks, maybe these sort of groups we see represent contacts over a single day, and the vertices in each day are very sparsely connected with the other vertices from the other days... It is interesting how the days are even still temporally connected through these paths. I guess these low degree nodes could be the organizers (but probably too many to explain it), hrmmm.. Low degree nodes seem to hold the entire reachability-graph together.
  \label{fig:loss}
    \vspace{-5mm}
\end{figure*}



%The reachability graphs are also useful to analyze the temporal properties.
%The reachability graphs may also be useful for analyzing the temporal properties or the overall communication capabilities of the time-evolving graph.
%
% or providing bounds on the transfer of information or communication capabilities of the time-evolving graph.
%Reachability graph reveals the connectivity properties of the temporal graph from which they arise.
%%Note that the reachability graph reveals the connectivity properties of the temporal graph from which they arise.
%Moreover, these graphs provide bounds on the communication capabilities of the time-evolving graph.
%
%
%The temporal reachability graphs reveal the temporal connectivity of the time-evolving graphs from which they arise.
%Moreover, these graphs provide bounds on the communication capabilities of the time-evolving graph.


%Both problems are known to be NP-hard.
%We briefly define the strong reachability graph below.
%
%It has been shown that finding a temporal SCC in $\mathcal{G}$ is equivalent to finding maximal cliques in the reachability graph $\mathcal{R}_s$ \cite{bhadra2003complexity}.
%Let us note that enumerating all of the tSCC's in $\mathcal{G}$ is as difficult as enumerating all the maximal cliques in $\mathcal{R}_s$. 
%
%%We posit that the maximum tSCC is the one of main interest as most practical applications such as routing 
%
%We move from the notion of time-evolving graphs to that of reachability graphs and show that solving
%The transformation from the evolving graph $\mathcal{G}$ to the reachability graph $\mathcal{R}$ allows us to solve the problem of finding the SCC's in $\mathcal{G}$ by solving the equivalent problem of finding the maximal cliques in $\mathcal{R}$.
%
%%The transformation from the evolving graph $\mathcal{G}$ into the static undirected strong reachability graph $\mathcal{R}_s$ allows us to use well-known results for the clique problem.
%%Listing all maximal cliques of a graph takes exponential time.
%%In this work, we focus on computing the $\textbf{maximum clique}$ in $\mathcal{R}_s$ which corresponds to the largest strongly connected component in $\mathcal{G}$.









%\noindent \textit{Approximating the Largest Temporal SCC}.
%we may also approximate the temporal SCC using the heuristic maximum clique method.
%\noindent \textit{Computing the Exact Largest Temporal SCC}.




%some properties of the reachability graph...


%Moreover, Whitbeck et al. defines entire families of reachability graphs with various properties.
%Each type could be adapted for our purposes.
%In this paper, we focus on computing max cliques from large realistic graphs, and thus we allow the reachability graph to become dense over time, without considering duration (as this can be tuned for specific applications).
%The simple method used for computing the reachability graph is given in Algorithm~\ref{alg:reachability}.
%For this purpose algorithm~\ref{alg:reachability} for a sim
% the on the case when the reachability graph becomes 
%However, the focus of our paper is not on reachability graphs, but computing max cliques and temporal SCC's from large graphs.
%Nevertheless, since this paper focuses on computing max cliques from large graphs, we only consider the

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Max Clique methods
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%todo: discuss the two methods, when to use one over the other, benefits of heuristic, etc... 
%todo: also analyze/discuss the above empirically












%\subsubsection{Approximating Temporal Components}

%\subsection{Exact and Approximate Solutions for Largest Temporal SCC}
%\subsection{Approximating the Largest tSCC}
%\subsection{Computing the Reachability Graph}


%Suppose, there exists a temporal path $u \leadsto w$ 
%If there exists a directed edge from u to w in $\mathcal{R}$, but not an edge from w to u, then information can only flow from u to w, but not from w to u.
%In essence, this means that at some time $t$, information flowed from u to w, and at $t+1$ the information can also flow to any contacts from $w$ to any other vertex.
%
%todo: What are the correlations between symmetric and asymmetric edges from any given vertex?







%dividing the vertices by the number of computers and assigning one or more computers to solve each subproblem. 
%The, since for each node, we can call a function \textsf{Reach(u,t)} and it returns a list of nodes with whom it can reach.


%The max clique procedure is fundamental to finding connected components on evolving graphs.
%Use max clique procedure to find temporal components.


%Moreover, the reachability graph can be used to investigate the properties of temporal graphs.

%and show that computing max cliques fast is fundamental to finding the largest connected component in an evolving graph.

%Therefore, we can solve the maximum clique problem in $\mathcal{R}$ using the fast maximum clique methods.
%The exact maximum clique algorithm offers a
%use our fast max clique algorithm or the extremely fast heuristic for 


%However, most importantly, the problem of finding a SCC in $\mathcal{G}$ is equivalent to finding cliques in $\mathcal{R}_s$.

% the fast maximum clique algorithm to compute the maximum temporal strongly connected component.
%The relationship between the tSCC's in $\mathcal{G}$ and the maximal-cliques in $\mathcal{R}_s$ allows us to use the fast maximum clique algorithm to compute the maximum temporal strongly connected component.
%In general, there may be multiple maximum tSCC's in $\mathcal{G}$ and our methods can find them by simplying removing the last found maximum clique from $\mathcal{R}_s$ and iterating.




%\begin{figure}
%\begin{center}
%\begin{minipage}
%\begin{algorithm}[H]
%\IncMargin{-1mm}
%\RestyleAlgo{ruled}
%\begin{algorithmic}[1]
%%\begin{algorithm}[t!]
%\caption{Exact algorithm for Maximum Temporal SCC}
%\label{alg:tscc}
%%\SetKwComment{Comment}{//}{}
%%\SetSideCommentRight
%\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
%\KwIn{\hspace{1mm} Time-evolving Graph $\mathcal{G} = (V,E,\mathcal{T})$}
%\KwOut{Maximum tSCC}
%\medskip
%\textbf{procedure} \textsc{MaxTSCC}($\mathcal{G} = (V,E,\mathcal{T})$) \\
%$\mR = $\textsc{Reach}($\mathcal{G}$)\\
%%$R_s \equiv \{\forall(u,w) : [(u,w) \wedge (w,u)] \in \mR \\}$
%$\mR_s = \mR \wedge \mR^T$ \scriptsize\tcp*[f]{\hspace{-3mm} symmetrize}\normalsize \\
%$k$ = \textsc{MaxCore}($\mR_s$)  \scriptsize\tcp*[f]{\hspace{-3mm} max k-core lower-bound}\normalsize \\
%$\mathcal{C}_{max}$ = \textsc{MaxClique}($\mathcal{R}_s = (V_s, E_s)$, $k_{max}$)
%%\end{algorithm}
%\end{algorithmic}
%
%\RestyleAlgo{plain}
%\IncMargin{-0mm}
%%\restylealgo{} \nocaptionofalgo
%%\NoCaptionOfAlgo
%%\begin{algorithm}[t!]
%\begin{algorithmic}[1]
%\vspace{-6mm}
%%\NoCaptionOfAlgo
%\SetAlgoNoLine
%\SetKwInOut{Sub}{\hspace{-4mm} \small \textsf{\textit{Subroutine}}}
%\Sub{}
%\smallskip
%\textbf{procedure} \textsc{Reach}($\mathcal{G} = (V,E,\mathcal{T})$) \\
%$E=[e(t_{max}),...,e(t_0)]$  \scriptsize\tcp*[f]{\hspace{-3mm} sort in reverse time order}\normalsize \\
%$\mR = \eye$ \scriptsize\tcp*[f]{\hspace{-3mm} current reachability matrix}\normalsize \\
%\For{$(i,j,t) \in E$} %\tiny\tcp*[f]{\tiny reachable vertices from $i$ and $j$}\normalsize \\
%{
%	$\mathcal{P} \equiv [k : (R_{i,k} \vee R_{j,k}) \notin \{i,j\} ] $ \\
%	\For{$k \in \mathcal{P}$}{
%			$R_{i,k} = 1$\\
%	}
%}
%\vspace{-5mm}
%%\end{algorithm}
%\end{algorithmic}
%\end{algorithm}
%\end{minipage}
%\end{center}
%\end{figure}





%Most importantly, the problem of finding a temporal SCC in $\mathcal{G}$ has been shown to be equivalent to finding cliques in the reachability graph $\mathcal{R}_s$ \cite{bhadra2003complexity}.
%As a consequence, the largest temporal connected component of $\mathcal{G}$ corresponds to the maximal clique of $\mathcal{R}$.
%Therefore, we transform the evolving graph into a reachability graph, and use our fast max clique algorithm for computing the largest temporal SCC (also sometimes referred to as the giant temporal component).
%%Since the temporal SCC's can share vertices
%
%Not surprisingly, the directionality of time offers an exact, yet efficient single-pass algorithm for computing the reachability graph.
%We discuss this next.



%Let us note that the case where edges last for only a duration is
%Let us note that if the edges last for only a duration $\delta t$, then computing the TSCC becomes much easier, since edges and thus possible temporal paths are removed. 
%Nevertheless, our methods are general enough to handle this specific case.




%RESULTS
%%%%%%%%%
%Looking at the results, the max k-core seems to provide a good lower-bound in the case of the reachability graphs.
%In most of the cases, if we had given as input the max k-core to the heuristic algorithm, it would have provided us with a more accurate maximum clique (meaning that the size of the max clique given by the heuristic algorithm is always lower than the max k-core on the reachability graphs).
%However, even though the kcore is linear to compute, it would still probably take longer than the heuristic (at least on some graphs).
%For instance, the heuristic only took 38 seconds, it is hard to imagine the kcore beating that time. But this might be something to mention in the paper, that if the additional time doesn't matter too much, then for denser graphs, providing the k-core as a lower-bound provides a more accurate solution in less time than the exact method.

%
%Temporal Strongly Connected Components (TSCC). We compute the temporal reachability matrix $\mR$ then $R_{strong} = \mR\&\mR^T$, which is given as input into the fast max clique procedure.






\begin{table}[t!]
\caption{\textbf{Max Cliques in Real Data}. }
\vspace{1mm}
\label{table:mc_data}
\centering\small
\begin{tabular}{l !{\vrule width 0.1mm} cc!{\vrule width 0.3mm}rr}
\TT  &\multicolumn{2}{c!{\vrule width 0.3mm}}{\small \textbf{Max Clique Size}} & \multicolumn{2}{c}{\small\textbf{Time} (seconds)}\\ 
\cline{2-5}
\TT \textbf{Graph} &  \textsf{\textbf{Exact}}  & \textsf{\textbf{Heur}} & \textsf{\textbf{Exact}} & \textsf{\textbf{Heur}} \\ 
\noalign{\hrule height 0.3mm}
\TT
   \textsc{yeast} & 6 & 6 & 0.03 s  & 0.03 s\\ 
   \textsc{celegans} & 9 & 8 & 0.02 s  & 0.03 s\\ 
\cline{1-5}
\TT
   \textsc{reality} & 5 & 5 & 0.03 s  & 0.04 s\\ 
   \textsc{wiki-vote} & 7 & 6 & 0.03 s  & 0.03 s\\ 
   \textsc{enron-only} & 8 & 7 & $<$ 0.01 s  & $<$ 0.01 s\\ 
   \textsc{wiki-talk} & 15 & 12 & 3.83 s  & 0.12 s\\ 
   \textsc{enron-large} & 20 & 16 & 1.1 s  & 0.05 s\\ 
   \textsc{mathscinet} & 25 & 25 & 0.07 s  & 0.08 s\\ 
   \textsc{ca-condmat} & 26 & 26 & 0.02 s  & 0.02 s\\ 
   \textsc{ca-astroph} & 57 & 57 & 0.14 s  & 0.07 s\\ 
   \textsc{ca-hepph} & 239 & 239 & 0.05 s  & 0.8 s\\ 
\cline{1-5}
\TT
   \textsc{infect-hyper} & 15 & 13 & 0.03 s  & 0.03 s\\ 
   \textsc{infect-dubli} & 16 & 16 & 0.02 s  & 0.03 s\\ 
\cline{1-5}
\TT
   \textsc{amazon} & 6 & 6 & 0.03 s  & 0.02 s\\ 
\cline{1-5}
\TT
   \textsc{roadnet-pa} & 4 & 4 & 0.13 s  & 0.21 s\\ 
   \textsc{roadnet-ca} & 4 & 4 & 0.29 s  & 0.49 s\\ 
\cline{1-5}
\TT
   \textsc{twitter-cope} & 4 & 4 & 0.03 s  & 0.03 s\\ 
   \textsc{retweet} & 4 & 4 & 0.03 s  & 0.04 s\\ 
   \textsc{polblogs} & 9 & 9 & 0.04 s  & 0.04 s\\ 
   \textsc{youtube} & 16 & 12 & 10.37 s  & 0.79 s\\ 
   \textsc{retweet-craw} & 13 & 13 & 1.9 s  & 0.51 s\\ 
   \textsc{epinions} & 16 & 14 & 0.16 s  & 0.01 s\\ 
   \textsc{slashdot} & 26 & 21 & 10.57 s  & 0.09 s\\ 
   \textsc{flickr} & ? & 36 & ? s  & 1.39 s\\ 
   \textsc{orkut} & 47 & 43 & 20650 s  & 21.72 s\\ 
   \textsc{livejournal} & ? & 214 & ? s  & 2.06 s\\ 
\cline{1-5}
\TT
   \textsc{fb-forum} & 4 & 4 & 0.03 s  & 0.03 s\\ 
   \textsc{fb-messages} & 5 & 5 & 0.03 s  & 0.02 s\\ 
\cline{1-5}
\TT
   \textsc{duke} & 34 & 29 & 229 s  & 0.1 s\\ 
   \textsc{berkeley} & 42 & 36 & 64.79 s  & 0.17 s\\ 
   \textsc{penn} & 44 & 42 & 30.86 s  & 0.6 s\\ 
   \textsc{stanford} & 51 & 46 & 769.31 s  & 0.37 s\\ 
   \textsc{texas} & 51 & 43 & 6982.83 s  & 0.78 s\\ 
\cline{1-5}
\TT
   \textsc{gowalla} & 29 & 29 & 1.68 s  & 0.41 s\\ 
   \textsc{brightkite} & 37 & 33 & 4.62 s  & 0.03 s\\ 
\cline{1-5}
\TT
   \textsc{p2p-gnutella} & 4 & 4 & 0.06 s  & 0.02 s\\ 
   \textsc{iptrace-redu} & 5 & 5 & 0.19 s  & 0.04 s\\ 
   \textsc{iptrace} & 8 & 6 & 106.56 s  & 1.51 s\\ 
   \textsc{internet-as} & 16 & 10 & 0.33 s  & 0.07 s\\ 
   \textsc{routers-rf} & 16 & 15 & 0.02 s  & 0.03 s\\ 
   \textsc{whois} & 58 & 50 & 11642 s  & 0.1 s\\ 
   \textsc{as-skitter} & 67 & 61 & 2084.43 s  & 5.39 s\\ 
\cline{1-5}
\TT
   \textsc{web-google} & 33 & 33 & 0.03 s  & 0.13 s\\ 
   \textsc{wikipedia} & 34 & 34 & 4.48 s  & 0.13 s\\ 
\bottomrule
\end{tabular}
\end{table}

\begin{table}[t!]
\caption{\textbf{Max Cliques in Real Data}. }
\vspace{1mm}
\label{table:mc_data}
\centering\small
\begin{tabular}{l !{\vrule width 0.1mm} cc!{\vrule width 0.3mm}rr}
\TT  &\multicolumn{2}{c!{\vrule width 0.3mm}}{\small \textbf{Max Clique Size}} & \multicolumn{2}{c}{\small\textbf{Time} (seconds)}\\ 
\cline{2-5}
\TT \textbf{Graph} &  \textsf{\textbf{Exact}}  & \textsf{\textbf{Heur}} & \textsf{\textbf{Exact}} & \textsf{\textbf{Heur}} \\ 
\noalign{\hrule height 0.3mm}
\TT
   \textsc{\scriptsize \#assad} & 2 & 2 & 0.02 s  & 0.03 s\\ 
   \textsc{\scriptsize \#barackobama} & 2 & 2 & 0.03 s  & 0.03 s\\ 
   \textsc{\scriptsize \#damascus} & 2 & 2 & 0.03 s  & 0.02 s\\ 
   \textsc{\scriptsize \#dash} & 2 & 2 & 0.03 s  & 0.02 s\\ 
   \textsc{\scriptsize \#gmanews} & 2 & 2 & 0.02 s  & 0.03 s\\ 
   \textsc{\scriptsize \#gop} & 2 & 2 & 0.03 s  & 0.03 s\\ 
   \textsc{\scriptsize \#israel} & 2 & 2 & 0.02 s  & 0.03 s\\ 
   \textsc{\scriptsize \#justinbieber} & 2 & 2 & 0.03 s  & 0.03 s\\ 
   \textsc{\scriptsize \#lebanon} & 2 & 2 & 0.02 s  & 0.02 s\\ 
   \textsc{\scriptsize \#libya} & 2 & 2 & 0.02 s  & 0.03 s\\ 
   \textsc{\scriptsize \#lolgop} & 2 & 2 & 0.03 s  & 0.03 s\\ 
   \textsc{\scriptsize \#mittromney} & 2 & 2 & 0.03 s  & 0.03 s\\ 
   \textsc{\scriptsize \#obama} & 2 & 2 & 0.03 s  & 0.03 s\\ 
   \textsc{\scriptsize \#oman} & 2 & 2 & 0.03 s  & 0.03 s\\ 
   \textsc{\scriptsize \#onedirection} & 2 & 2 & 0.03 s  & 0.03 s\\ 
   \textsc{\scriptsize \#p2} & 2 & 2 & 0.03 s  & 0.03 s\\ 
   \textsc{\scriptsize \#qatif} & 2 & 2 & 0.03 s  & 0.03 s\\ 
   \textsc{\scriptsize \#tcot} & 2 & 2 & 0.04 s  & 0.03 s\\ 
   \textsc{\scriptsize \#tlot} & 2 & 2 & 0.03 s  & 0.02 s\\ 
   \textsc{\scriptsize \#uae} & 2 & 2 & 0.02 s  & 0.02 s\\ 
   \textsc{\scriptsize \#voteonedirec} & 2 & 2 & 0.03 s  & 0.03 s\\ 
   \textsc{\scriptsize \#alwefaq} & 3 & 3 & 0.03 s  & 0.03 s\\ 
   \textsc{\scriptsize \#bahrain} & 3 & 3 & 0.03 s  & 0.02 s\\ 
   \textsc{\scriptsize \#http} & 3 & 3 & 0.04 s  & 0.02 s\\ 
   \textsc{\scriptsize \#ksa} & 4 & 4 & 0.03 s  & 0.02 s\\ 
   \textsc{\scriptsize \#saudi} & 4 & 4 & 0.03 s  & 0.02 s\\ 
\bottomrule
\end{tabular}
\end{table}





==> table_tscc_retweets.tex <==
\begin{tabular}{l !{\vrule width 0.1mm} cc!{\vrule width 0.3mm}rr}
\TT  &\multicolumn{2}{c!{\vrule width 0.3mm}}{\small \textbf{Max Clique Size}} & \multicolumn{2}{c}{\small\textbf{Time} (seconds)}\\ 
\cline{2-5}
\TT \textbf{Graph} &  \textsf{\textbf{Exact}}  & \textsf{\textbf{Heur}} & \textsf{\textbf{Exact}} & \textsf{\textbf{Heur}} \\ 
\noalign{\hrule height 0.3mm}
\TT
\bottomrule
\end{tabular}

